Noise is All You Need: Private Second-Order Convergence of Noisy SGD

Private optimization is a topic of major interest in machine learning, with differentially private stochastic gradient descent (DP-SGD) playing a key role in both theory and practice. Furthermore, DP-SGD is known to be a powerful tool in contexts beyond privacy, including robustness, machine unlearning, etc. Existing analyses of DP-SGD either make relatively strong assumptions (e.g., Lipschitz continuity of the loss function, or even convexity) or prove only first-order convergence (and thus might end at a saddle point in the non-convex setting). At the same time, there has been progress in proving second-order convergence of the non-private version of ``noisy SGD'', as well as progress in designing algorithms that are more complex than DP-SGD and do guarantee second-order convergence. We revisit DP-SGD and show that ``noise is all you need'': the noise necessary for privacy already implies second-order convergence under the standard smoothness assumptions, even for non-Lipschitz loss functions. Hence, we get second-order convergence essentially for free: DP-SGD, the workhorse of modern private optimization, under minimal assumptions can be used to find a second-order stationary point.

==> checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See~\Cref{thm:combine_main} and \Cref{ssec:high_prob}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All assumptions are stated in \Cref{sec:pre}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All assumptions are stated in \Cref{sec:pre}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See \Cref{sec:experiments,app:experimental_details}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All data is public, and we plan to release the code in the future. For reviewing purposes, the code is provided in the supplementary.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We use the datasets as is. The algorithm is as described in the paper. Additional details are in \Cref{app:experimental_details}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: For all plots, the captions explain what the data points and the error bars mean. We report the mean over the $10$ runs as well as minimum and maximum values over the runs.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We specified the training environment.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper conforms with the Code of Ethics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We don't expect the paper to have a direct societal impact
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: None of the outlined scenarios applies
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We cite all the datasets used in the paper.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper doesn't release new assets
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing nor research with human subjects
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing nor research with human subjects
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}



==> failed_clipping_proof_convergence.tex <==
\section{Convergence Proof}

\begin{assumption}
    \label{ass:main_new}
    The objective function $f$ and the component functions $f_i$ satisfy the following conditions.
    \begin{enumerate}
        {\color{green}\item (Boundedness) 
            There exists $\fmax$ such that $\fmax > f(\x{0}) - f(\vx^*)$.}
        {\color{green}\item (Smoothness) $f$ is $L$-smooth, i.e. $\norm{\nabla f(\vx) - \nabla f(\vy)} \le L \norm{\vx - \vy}$ for all $\vx, \vy \in \R^d$.
            Consequently, $f$ is also $L$-smooth.}
        {\color{green}\item (Lipschitz Hessian) The objective function $f$ has a $\rho$-Lipschitz Hessian, i.e. $\norm{\nabla^2 f(\vx) - \nabla^2 f(\vy)} \le \rho \norm{\vx - \vy}$ for all $\vx, \vy \in \R^d$.}
        {\color{red}\item (Relaxed Stochastic variance) The stochastic variance is bounded as follows: $\avg_{i=1}^N \norm{\nabla f_i(\vx) - \nabla f(\vx)}^2 \le \sigma_1^2 \SqrNorm{\nabla f(\vx)} + \sigma_2^2$.}
    \end{enumerate}
\end{assumption}

\todo{Rewrite}
\begin{assumption}
    {\color{red}No nSG assumption.}
\end{assumption}
\begin{assumption}
    {\color{red}Clipping.}
\end{assumption}

\label{app:convergence_proof}

\todo{Mention that mostly follows Jin et al.}

\begin{definition}
    \label{def:notation}    
    We introduce the following auxiliary notation.
    \begin{itemize}
        \item Let $\fullVar = \sigma^2 / B + d \Delta^2$ be the total noise variance.
        \item Let $\clipC$ be the clipping threshold. Can be set to infinity when there is no clipping.
        \item Let $\clip{t}$ be clipping scaling at iteration $t$: $\clip{t} = \max(1, \|\nabla f_{\batch{t}}(\x{t})\| / \clipC)$.
        \item Let $\nabla \fclip_{\batch{t}}(\x{t})$ be clipped stochastic gradient at iteration $t$: $\nabla \fclip_{\batch{t}}(\x{t}) = \nabla f_{\batch{t}}(\x{t}) / \clip{t}$.
    \end{itemize}
\end{definition}

\begin{definition}
    \label{def:params}
    Our choice of parameters is the following ($\cstep, \cit, \crad, \cf$ hide polylogarithmic dependence on all parameters):
    \begin{equation*}
        \begin{aligned}
            \text{Step size} && \step &= \cstep \min\pars{\frac{\alpha^2}{L (1 + \tsigma^2)}, \frac{\fmax}{L \tsigma^2}} \\
            \text{Total number of iterations} && T &= \frac{64\fmax}{\step \alpha^2} \\
            \text{Iterations required for escaping} && \escIter &=  \cit \frac {1} {\step \sqrtra} \\
            \text{Escaping radius} && \escRad &= \crad \sqrt {\alpha / \rho} \\
            \text{Objective decrease after successful escaping} && \df &= \cf \sqrtfacr
            % \text{Noise standard deviation} && r &= \cnoise \frac \alpha {\sqrt{\gradLip \step}}
        \end{aligned}
        % \label{eq:params}
    \end{equation*}
\end{definition}
Intuitively, the parameters are chosen as follows.
Assume that the current point is $\vzero$ and the function is quadratic, i.e. $f(\vx) = \vx^T H \vx$.
If $\vx$ is a saddle point, then we know that the smallest eigenvalue of $H$ is $-\eigen < -\sqrtra$ with the corresponding eigenvector $\vv_1$.
Then, the largest function decrease would be in the direction of $\vv_1$, and this direction can be found using power method for the appropriate matrix.
But, if we look at the gradient descent update:
\[
    \x{t+1}
    = \x{t} - \step \nabla f(\x{t})
    = \x{t} - \step 2 H \x{t}
    = (\id - \step 2 H) \x{t},
\]
we see that for quadratic functions, gradient descent is exactly the power method for the matrix $\id - \step 2H$, which has the same eigenvectors as $H$.\footnote{More complicated, but similar logic works for gradient descent with clipping}
The eigenvalue $-\eigen$ of $H$ corresponds to the eigenvalue $1 + 2 \step \eigen$ of $1 - \step 2 H$, which is the largest (by absolute value) eigenvalue when $\step \le 1/L$.
Note that power method requires some initial randomness, which explains while randomness is required to escape from saddle points.

The above intuition motivates the choice of parameters.
\begin{itemize}
    \item
        \textbf{Escaping radius $\escRad$}. Since in general the function is not necessarily quadratic, we want to guarantee that the Hessian doesn't change excessively.
        More specifically, we want the smallest eigenvalue to be at most $-\eigen / 2$ for the entire escaping procedure.
        By the Hessian-Lipschitz property $\|\nabla^2 f(\vx) - \nabla^2 f(\vy)\| \le \rho \|\vx - \vy\|$, if we work in the radius $\escRad = \eigen /(2\rho)$, then for any point within the radius $\escRad$ of the initial point, the smallest eigenvalue is at most $-\eigen + \eigen / 2 = -\eigen / 2$.
        When $\eigen > \sqrtra$, we can lower-bound $\escRad$ as $\sqrtra / (2\rho) = \sqrt{\alpha / (4\rho)}$.
    \item
        \textbf{Number of iterations required for escaping $\escIter$}.
        After $t$ iterations, the length of $\x{t}$ along the $\vv_1$ direction is $(1 + \step \eigen)^t \approx e^{t / (\step \eigen)}$.
        Hence, we reach the boundary of the ball of radius $\escRad$ after $(t \log \escRad) / (\step \eigen)$ iterations.
    \item
        \textbf{Function change after escaping $\df$}.
        Since we are working inside the ball of size $\escRad$, the best objective improvement $\df$ we can aim for is achievable by moving by $\escRad \vv_1$.
        This improves the objective by approximately $\escRad^2 \eigen$, which, by the choice of the parameters can be lower-bounded as $\alpha / \rho \cdot \sqrtra = \sqrt{\alpha^3 / \rho}$.
    \item
        \textbf{Total number of iterations $T$}. Every $\escIter$ iterations we improve objective by $\df$.
        Since the total objective improvement cannot exceed $\fmax$, the maximum number of iterations is
        \[
            \frac{\fmax \escIter}{\df}
            \le \frac{\fmax}{(\step \sqrtra)\sqrt{\alpha^3 / \rho}}
            = \frac{\fmax}{\step \alpha^2}
        \]
\end{itemize}

\begin{lemma}[Descent Lemma]
    \label{lem:descent}
    Assume that $\step < 1/L$, for any $t_0$ and $t$.
    Then, with probability at least $1 - \tdelta$, for some constant $c$:
    \[
        f(\x{t_0}) - f(\x{t_0 + t})
        \ge \frac{\step}{8} \sum_{\tau=t_0}^{t_0 + t - 1} \norm{\nabla f(\x{\tau})}^2 - c \step \tsigma^2 (\step L t + \logErr)
        .
    \]
\end{lemma}

\begin{proof}
    W.l.o.g., we consider $t_0 = 0$.
    Let $\sgdNoise{\tau} = \nabla f_{\batch{t}}(\x{\tau}) - \nabla f(\x{\tau})$ be the stochastic noise at iteration $\tau$.
    By the folklore Descent Lemma,
    \begin{align*}
        f(\x{\tau}) - f(\x{\tau+1})
        % \ge \step \sum_{\tau=0}^{t-1} \InnerProd{\nabla f(\x{\tau}), \nabla f_{\batch{t}}(\x{\tau})}
            % - \frac{L}{2} \SqrNorm{\x{}}
        &\ge \step \InnerProd{\nabla f(\x{\tau}), \nabla \fclip_{\batch{t}}(\x{\tau})}
            - \frac{L}{2} \SqrNorm{\x{\tau + 1} - \x{\tau}} \\
        &= \step \InnerProd{\nabla f(\x{\tau}), \frac{\nabla f(\x{\tau}) + \sgdNoise{\tau}}{\clip{\tau}} + \ourNoise{\tau}}
            - \frac{L\step^2}{2} \SqrNorm{\frac{\nabla f(\x{\tau}) + \sgdNoise{\tau}}{\clip{\tau}} + \ourNoise{\tau}} \\
        &\ge \frac{\step}{\clip{t}} \SqrNorm{\nabla f(\x{\tau})}
            + \step \InnerProd{\nabla f(\x{\tau}), \frac{\sgdNoise{\tau}}{\clip{\tau}} + \ourNoise{\tau}}
            - \frac{\step^2 L}{2} \pars{\frac{3}{2} \SqrNorm{\frac{\nabla f(\x{\tau})}{\clip{\tau}}} + 3 \SqrNorm{\frac{\sgdNoise{\tau}}{\clip{\tau}} + \ourNoise{\tau}}}
        % &= \step \InnerProd{\nabla f(\x{\tau}), \nabla f(\x{\tau}) + \sgdNoise{\tau}}
        %     - \frac{L\step^2}{2} \SqrNorm{\nabla f(\x{\tau}) + \sgdNoise{\tau}} \\
        ,
    \end{align*}
    where we used inequality $\|a + b\|^2 \le (1 + \nu) \|a\|^2 + (1 + 1/\nu)\|b\|^2$ for $\nu = 1/2$.
    By telescoping,
    \begin{align*}
        f(\x{0}) - f(\x{t})
        &\ge \frac{\step}{4} \sum_{\tau=0}^{t-1} \frac{\SqrNorm{\nabla f(\x{\tau})}}{\clip{\tau}}
            + \step \sum_{\tau=0}^{t-1} \InnerProd{\nabla f(\x{\tau}), \frac{\sgdNoise{\tau}}{\clip{\tau}} + \ourNoise{\tau}}
            - \frac{3 \step^2 L}{2} \sum_{\tau=0}^{t-1} \SqrNorm{\frac{\sgdNoise{\tau}}{\clip{\tau}} + \ourNoise{\tau}}
        % &= \step \InnerProd{\nabla f(\x{\tau}), \nabla f(\x{\tau}) + \sgdNoise{\tau}}
        %     - \frac{L\step^2}{2} \SqrNorm{\nabla f(\x{\tau}) + \sgdNoise{\tau}} \\
    \end{align*}
    %
    Using a concentration inequality for nSG variables, with probability at least $1 - \tdelta$ for some constant $c$ we have
    \todo{Handle that}
    \[
        \abs{\step \sum_{\tau=0}^{t-1} \InnerProd{\nabla f(\x{\tau}), \sgdNoise{\tau} + \ourNoise{\tau}}}
        \le \frac{\step}{8} \sum_{\tau=0}^{t-1} \SqrNorm{\nabla f(\x{\tau})} + c \step \fullVar^2 \logErr
    \]
    \todo{Give reference}
    \todo{Avoid norm-subGaussian}
    For the last term, with probability at least $1 - \tdelta$ we have
    \[
        \frac{3 \step^2 L}{2} \sum_{\tau=0}^{t-1} \SqrNorm{\sgdNoise{\tau}}
        \le c \step^2 L \fullVar^2 (t + \logErr).
    \]
    Combining the above inequalities and using $\step \le 1/L$ finishes the proof.
    % \todo{TODO}
\end{proof}

\subsection{Large Gradient Case}

\todo{Get rid of frac in the text}

The first application of the Descent Lemma is to bound the number of iterations when the gradient is large.
\begin{lemma}
    \label{lem:quarter_large_grad}
    When $T \ge \frac{64 \fmax}{\step \alpha^2}$ and other parameters are as in \Cref{def:params}, the number of iterations $t$ with $\|\nabla f(\x{t})\| \ge \alpha$ is at most $\nicefrac T4$.
\end{lemma}

\begin{proof}
    For the sake of contradiction, assume that the number of points $\x{t}$ with $\|\nabla f(\x{t})\| \ge \alpha$ is greater than $\nicefrac T4$.
    Then, by the Descent Lemma we have
    \begin{align*}
        f(\x{0}) - f(\x{T})
        &\ge \frac{\step}{8} \sum_{\tau=0}^{T - 1} \norm{\nabla f(\x{\tau})}^2 - c \step \tsigma^2 (\step L T + \logErr) \\
        &\ge \frac{\step T \alpha^2}{32}  - c \step T \cdot \tsigma^2 \pars{\step L + \frac{\logErr}{T}}
    \end{align*}
    We will show that the right-hand side is at least $\fmax$, leading to contradiction.
    For that, it suffices to guarantee that $\frac{\step T \alpha^2}{32} \ge 2\fmax$ and $c \step T \cdot \tsigma^2 \pars{\step L + \frac{\logErr}{T}} \le \fmax$.
    The former condition is satisfied by our choice of $T$, and substituting the bound on $\fmax$ into the latter condition shows that it suffices to prove
    \[
        64 c \tsigma^2 \pars{\step L + \frac{\step \alpha^2 \logErr}{64 \fmax}} \le \alpha^2
    \]
    It suffices to bound each term with $\alpha^2 / 2$, which is satisfied for
    \begin{align*}
        \step &\le \frac{\alpha^2}{128 \cdot c \tsigma^2 L} \\
        \step &\le \frac{\fmax\logErr}{2 \cdot c \tsigma^2 L}
    \end{align*}
    Both of these conditions are satisfied by our choice of $\step$, with the appropriate choice of $\cstep$.
\end{proof}




\subsection{Escaping From Saddle Points}

The Descent Lemma also implies the following result, which upper-bounds the distance change in terms of the objective changes.
Its \Cref{cor:i_or_l} states that, if after a bounded number of iterations the point moves far from the original point, then the objective value sufficiently decreases.
%
\begin{lemma}[Improve or localize]
    \label{lem:improve_or_localize}
    For any $t_0$ and $t$, with probability at least $1 - \tdelta$, for some constant $c$:
    \begin{align*}
        \SqrNorm{\x{t_0 + t} - \x{t_0}}
        \le c \step t \pars{(f(\x{t_0}) - f(\x{t_0 + t}) + \step \tsigma^2 (\step L t + \logErr)}
    \end{align*}
\end{lemma}
%
\begin{proof}
    W.l.o.g. we consider the case when $t_0 = 0$.
    % By the Descent Lemma,
    % \[
    %     f(\x{0}) - f(\x{t})
    %     \ge \frac{\step}{8} \sum_{\tau=0}^{t - 1} \norm{\nabla f(\x{\tau})}^2 - c \step \tsigma^2 (\step L t + \logErr)
    % \]
    By the definition of $\x{\tau + 1}$, we have
    \begin{align*}
        \x{\tau} - \x{\tau + 1}
        = \step (\nabla f_{\batch{\tau}}(\x{\tau}) + \ourNoise{\tau})
        = \step (\nabla f(\x{\tau}) + \sgdNoise{\tau} + \ourNoise{\tau}),
    \end{align*}
    where $\sgdNoise{\tau} = \nabla f_{\batch{\tau}}(\x{\tau}) - \nabla f(\x{\tau})$ is stochastic gradient noise.
    By telescoping, we have:
    \begin{align*}
        \|\x{0} - \x{t}\|
        &= \step \norm{\sum_{\tau = 0}^{t - 1}(\nabla f(\x{\tau}) + \sgdNoise{\tau} + \ourNoise{\tau})}
    \end{align*}
    By Cauchy-Schwarz Inequality, we have:
    \begin{align*}
        \|\x{0} - \x{t}\|^2
        &\le 2 \step^2 \pars{\norm{\sum_{\tau = 0}^{t - 1}\nabla f(\x{\tau})}^2 + \norm{\sum_{\tau = 0}^{t - 1} (\sgdNoise{\tau} + \ourNoise{\tau})}^2} \\
        &\le 2 \step^2 \pars{t \sum_{\tau = 0}^{t - 1}\norm{\nabla f(\x{\tau})}^2 + \norm{\sum_{\tau = 0}^{t - 1} (\sgdNoise{\tau} + \ourNoise{\tau})}^2}
    \end{align*}
    \todo{Elaborate and avoid nSG}
    Since $\sgdNoise{\tau} + \ourNoise{\tau}$ is $\mathrm{nSG}(\fullVar^2)$, by applying concentration inequality for $\mathrm{nSG}$ variables, we have with probability at least $1 - \tdelta$:
    \begin{align*}
        \|\x{0} - \x{t}\|^2
        &\le 2 \step^2 \pars{t \sum_{\tau = 0}^{t - 1}\norm{\nabla f(\x{\tau})}^2 + c t \fullVar^2 \logErr}
    \end{align*}
    Finally, applying the Descent Lemma, we get
    \begin{align*}
        \|\x{0} - \x{t}\|^2
        &\le \step c t \pars{f(\x{0}) - f(\x{t}) + \step \fullVar^2 (\step L t + \logErr)}
    \end{align*}
    for some constant $c$.
\end{proof}


\begin{corollary}
    \label{cor:i_or_l}
    For the parameters chosen as in \Cref{def:params}, if for some $t \le \escIter$ we have $\SqrNorm{\x{t_0 + \tau} - \x{t_0}} \ge \escRad$, then $f(\x{t_0}) - f(\x{t_0 + \tau}) \ge \df$ with probability at least $1 - \tdelta$.
\end{corollary}
%
\begin{proof}
    From \Cref{lem:improve_or_localize}, we know that for some $c$:
    \begin{align*}
        f(\x{t_0}) - f(\x{t_0 + t})
        &\ge \frac{\escRad^2}{c \step \escIter} - \step \tsigma^2 (\step L \escIter + \logErr) \\
        &\ge \frac{\crad^2}{c \cit} \sqrtfacr - \step \tsigma^2 \pars{\frac{\cit L}{\sqrtra} + \logErr}
        % &\ge \frac{\SqrNorm{\x{t_0 + t} - \x{t_0}}}{c \step \escIter} - \step \tsigma^2 (\step L \escIter + \log 1/\fullVar)
    \end{align*}
    We want to guarantee that the right-hand side is at most $\df = \cf \sqrtfacr$.
    It suffices to guarantee that
    \begin{align*}
        \crad^2 / (c \cit) \ge 2 \cf \qquad \text{and} \qquad \step \tsigma^2 (\cit L / \sqrtra + \logErr) \le \cf \sqrtfacr.
    \end{align*}
    The former holds for the appropriate choice of $\crad$, $\cit$, and $\cf$, and the latter holds by choosing
    \[
        \step \le (\alpha^2 / L \tsigma^2) \cdot  \cf / \pars{\cit + \logErr},
    \]
    where we assumed $L \ge \sqrtra$, since otherwise any $\alpha$-FOSP is an $\alpha$-SOSP because $L$ is an upper bound on the absolute values of the Hessian.
\end{proof}

\begin{definition}[Coupling sequences]
    \label{def:coupling_sequence}
    Let $\vv_1$ be the eigenvector corresponding to the smallest eigenvalue of $\nabla^2 f(\x{t_0})$.
    The coupling sequences starting from $\x{t_0}$ are defined as follows:
    \begin{equation}
        \begin{aligned}
            \ourNoise{t_0+t} &\sim \mathcal{N}(0, \fullVar^2 \id) \\
                \tourNoise{t_0+t} &= \ourNoise{t_0+t} - 2 \InnerProd{ \vv_1, \ourNoise{t_0+t} } \vv_1  \\
                % \batch'_{t_0+t} &= \batch_{t_0+t}, \\
            \x{t_0 + t+1} &= \x{t_0+t} - \step (\nabla f_{\batch{t}}(\x{t_0 + t}) + \ourNoise{t_0 + t}) \\
            \tx{t_0 + t+1} &= \tx{t_0+t} - \step (\nabla f_{\batch{t}}(\tx{t_0 + t}) + \tourNoise{t_0 + t}) \\
            \sgdNoise{t_0 + t} &= \nabla f_{\batch{t}}(\x{t_0 + t}) - \nabla f(\x{t_0 + t}) \\
            \tsgdNoise{t_0 + t} &= \nabla f_{\batch{t}}(\tx{t_0 + t}) - \nabla f(\tx{t_0 + t}) \\
        \end{aligned}\nonumber
    \end{equation}
    %
    Note that:
    \begin{itemize}
        \item the artificial noise $\tourNoise{t_0 + t}$ has the opposite sign in direction $\vv_1$ compared with $\ourNoise{t_0 + t}$,
        \item the stochastic randomness ${\batch{t}}$ is the same for both sequences,\todo{Might be not required, but anyways makes things simpler to define}
        \item $\{\x{t_0 + t}\}_t$ and $\{\tx{t_0 + t}\}_t$ are sampled from the same distribution.
    \end{itemize}
    %
    We next define the difference between the coupling sequences:
    \begin{equation}
        \begin{aligned}
            \difourNoise{t} &= \xi_{t_0+t} - \xi'_{t_0+t} 
                = 2 \InnerProd{ \vv_1, \xi_{t_0+t} } \vv_1  \\
                % \batch'_{t_0+t} &= \batch_{t_0+t}, \\
            \difx{t_0 + t+1} &= \x{t_0+t} - \tx{t_0+t} \\
            \difsgdNoise{t_0 + t} &= \sgdNoise{t_0 + t} - \tsgdNoise{t_0 + t}
        \end{aligned}\nonumber
    \end{equation}
\end{definition}

% TODO (the rest is standard)

% SGD with variance $\sigma^2$ and batch size $B$, then the number of iterations to find an $\alpha$-FOSP ($\|\nabla f(\vx)\| < \alpha$) is $\frac{\sigma^2}{B \alpha^4}$.

From now on, we assume that we want to escape from point $\x{t_0}$ such that $\lmin(\nabla^2 f(\x{t_0})) < -\sqrtra$.
W.l.o.g. we assume $t_0 = 0$.
Let $H = \nabla^2 f(\x{0})$ be the Hessian of $f$ at point $\x{0}$, let $-\eigen = \lmin(H)$ be the smallest eigenvalue of $H$, and $\vv_1$ be the eigenvector corresponding to $-\eigen$.

\begin{lemma}
    For every $t$,
    \[
        \difx{t} = -\dif{t} - \sgdErr{t} -\quadErr{t},
    \]
    where
    \begin{align*}
        \dif{t} &= \step \sum_{\tau = 0}^{t - 1} (\id - \step H)^{t - 1 - \tau} \difourNoise{\tau} \\
        \sgdErr{t} &= \step \sum_{\tau = 0}^{t - 1} (\id - \step H)^{t - 1 - \tau} \difsgdNoise{\tau} \\
        \quadErr{t} &= \step \sum_{\tau = 0}^{t - 1} (\id - \step H)^{t - 1 - \tau} \hesInt{\tau} \difx{\tau},
            \quad \text{ where } \quad \hesInt{\tau} = \int_0^1  (\nabla^2 f(\psi \x{\tau} + (1 - \psi) \tx{\tau}) - H)\ d\psi
    \end{align*}
\end{lemma}
\begin{proof}
    Proof by induction.
    \begin{align*}
        \difx{t + 1}
        &= \difx{t} - \step (\difsgdNoise{t} + \difsgdNoise{t}) - \step (\nabla f(\x{t}) - \nabla f(\tx{t})) \\
        &= (1 - \step H) \difx{t} - \step (\difsgdNoise{t} + \difsgdNoise{t}) - \step (\nabla f(\x{t}) - \nabla f(\tx{t}) - H \difx{t})
    \end{align*}
    Using that $\nabla f(\x{t}) - \nabla f(\tx{t}) = \int_0^1  \nabla^2 f(\psi \x{\tau} + (1 - \psi) \tx{\tau}) \difx{\tau}\ d\psi$, by telescoping we complete the proof.
\end{proof}
%
In the following statements, the geometric series $\alpha_t^2 = \sum_{\tau = 0}^{t-1} (1 + \step \eigen)^{2 \tau}$ occurs frequently.
Intuitively, each iteration increases the distance approximately by a factor of $(1 + \step \eigen)$~-- the largest eigenvalue of matrix $I - \step H$.
The noise added at iteration $\tau$ gets amplified by $(1 + \step \eigen)^{t - \tau}$ by iteration $t$, and, if every iteration an independent noise of variance $\Delta^2$ is added, $\Delta^2 \alpha_t^2$ is the total variance of such a noise accumulated over the iterations.
%
\begin{lemma}
    \label{lem:alpha_beta}
    Let $\alpha_t = \sqrt{\sum_{\tau = 0}^{t-1} (1 + \step \eigen)^{2 \tau}}$ and $\beta_t = (1 + \step \eigen)^t / \sqrt{\step \eigen}$.
    If $\step \eigen < 1$, then $\alpha_t \le \beta_t$ for any $t$ and $\alpha_t \ge \beta_t / 3$ for $t \ge 2 / (\step \eigen)$.
\end{lemma}
\begin{proof}
    As a sum of geometric progression, we have
    \[
        \alpha_t^2
        = \frac{(1 + \step \eigen)^{2t} - 1}{(1 + \step \eigen)^2 - 1}
        = \frac{(1 + \step \eigen)^{2t} - 1}{\step \eigen (2 + \step \eigen)},
    \]
    and $\alpha_t^2 \le \beta_t^2$ follows immediately.
    On the other hand, for $t \ge 1 / (\step \eigen)$ we have $(1 + \step \eigen)^{2t} \ge 2$, and hence $(1 + \step \eigen)^{2t}  - 1 \ge (1 + \step \eigen)^{2t} / 2$.
    Finally, by our choice of the step size, we have $\step \eigen \le \step L \le 1$, and hence $2 + \step \eigen \le 3$.
    This implies $\alpha_t^2 \ge \beta_t^2 / 6$, finishing the proof.
\end{proof}

\begin{lemma}
    \label{lem:good_term}
    Let $\beta_t = (1 + \step \eigen)^t / \sqrt{\step \eigen}$.
    Then for any $t$ and $\tdelta$, for some constant $c$:
    \begin{align*}
        \P{\|\dif{t}\| \ge c \beta_t \step \Delta \sqrt{\logErr}} &\le \tdelta \\
        \P{\|\dif{t}\| \le \frac{\beta_t \step \Delta}{10}} &\le \frac 13
    \end{align*}
\end{lemma}
\todo{Check $\sqrt{\logErr}$}

\begin{proof}
    Since $\difourNoise{\tau} = 2\InnerProd{\ourNoise{\tau}, \vv_1} \vv_1$ and $\vv_1$ is an eigenvalue of $H$ corresponding to eigenvalue $-\eigen$, we have
    \[
        \dif{t}
        = \step \sum_{\tau = 0}^{t - 1} (\id - \step H)^{t - 1 - \tau} \difourNoise{\tau}
        = \pars{\step \sum_{\tau = 0}^{t - 1} (1 + \step \eigen)^{t - 1 - \tau} \InnerProd{\ourNoise{\tau}, \vv_1}} \vv_1
    \]
    Hence, $\dif{t}$ is a random variable which is parallel to $\vv_1$.
    % Hence, $\dif{t}$ is a Gaussian random variable along direction $\vv_1$ with variance $\step \sum_{\tau = 0}^{t - 1} (1 + \step \eigen)^{t - 1 - \tau} \InnerProd{\ourNoise{\tau}, \vv_1}$
    Since each $\ourNoise{t}$ is a Gaussian random variable with the covariance matrix $\Delta^2 \id$, each $\InnerProd{\ourNoise{t}, \vv_1}$ a Gaussian random variable with variance $\Delta^2$.
    Hence, $\dif{t}$ is also a Gaussian random variable, and
    \[
        \Var{\|\dif{t}\|}
        = \step \sum_{\tau = 0}^{t - 1} (1 + \step \eigen)^{\tau} \Delta^2
        = \Delta^2 \alpha_t^2
    \]
    The upper bound on $\|\dif{t}\|$ follows from \Cref{lem:alpha_beta} and standard concentration inequality for Guassians.
    The lower bound follows from inequality $\P{|X| \le \sigma a} \le a$ for $X \sim \mathcal{N}(0, \sigma^2)$ and any $a$.
\end{proof}

\todo{Be more careful with $\tdelta$}

\todo{Replace $\fullVar$ with $\Delta$ where required}

\todo{Propagate assumption $\Delta^2 \ge \sigma^2 / B$}

\begin{lemma}
    \label{lem:error_terms}
    Let $\mathcal{E}_t$ be the event ``$\|\x{0} - \x{\tau}\| < \escRad$ and $\|\x{0} - \tx{\tau}\| < \escRad$ for all $\tau < t$''.
    Then, when $\Delta^2 \ge \sigma^2 / B$, for some constant $c$ we have
    % \todo[inline]{Fix log error}
    \[
        \P{\mathcal{E}_\escIter
            \implies \max\nolimits_{\tau=0}^{\escIter - 1} \norm{\sgdErr{\tau} + \quadErr{\tau}}
            \le 
            c \beta_\tau \step \Delta \sqrt{\logErr}
        } \ge 1 - \escIter \tdelta
    \]
\end{lemma}
    
\begin{proof}
    By induction on $t$, we will prove that $\P{\mathcal{E}_t \implies \|\difx{t}\| \le c \step \Delta \beta_t} \le 1 - t\fullVar$ and
    \[
        \P{\mathcal{E}_t
            \implies \max\nolimits_{\tau=0}^{t - 1} \norm{\sgdErr{\tau} + \quadErr{\tau}}
            \le  c \beta_\tau \step \Delta \sqrt{\logErr}
        } \ge 1 - t \tdelta.
    \]
    Base case is $t=0$, in which case $\difx{0} = \vzero$.
    For the induction step, since $\difx{t} = -\dif{t} - \sgdErr{t} -\quadErr{t}$, we bound each term separately.
    \paragraph{Bounding $\dif{t}$}
    By \Cref{lem:good_term}, we have $\P{\|\dif{t}\| \ge c \beta_t \step \Delta \sqrt{\logErr}} \le \tdelta$.

    
    \paragraph{Bounding $\quadErr{t}$}
    Assuming $\mathcal{E}_t$, by the Hessian-Lipschitz property we have
    \begin{align*}
        \|\hesInt{\tau} \difx{\tau}\|
        &= \norm{\int_0^1  (\nabla^2 f(\psi \x{\tau} + (1 - \psi) \tx{\tau}) - H)\ d\psi \cdot \difx{\tau}} \\
        &\le 2 \rho \escRad \|\difx{\tau}\| \\
        &\le 2 \rho \escRad \cdot c \beta_\tau \step \Delta \sqrt{\logErr},
    \end{align*}
    %
    and we bound $\quadErr{t}$ as
    %
    \begin{align*}
        \|\quadErr{t}\|
        &= \norm{\step \sum_{\tau = 0}^{t - 1} (\id - \step H)^{t - 1 - \tau} \hesInt{\tau} \difx{\tau}} \\
        &\le \sum_{\tau = 0}^{t - 1} (1 + \step \gamma)^{t - 1 - \tau} 2 \rho \escRad \cdot c \beta_\tau \step \Delta \sqrt{\logErr} \\
        % &\le \sum_{\tau = 0}^{t - 1} (1 + \step \gamma)^{\tau} 2 \rho \escRad \cdot c \beta_t \step \fullVar^2 \sqrt{\logErr} \\
    \end{align*}
    Since $(1 + \step \gamma)^{t - 1 - \tau} \beta_\tau = \beta_{t-1}$,
    % \[
    %     \sum_{\tau = 0}^{t - 1} (1 + \step \gamma)^{\tau}
    %     = \frac{(1 + \step \gamma)^t - 1}{\step \gamma}
    %     \le \frac{\beta_t}{\sqrt{\step \gamma}},
    % \]
    we can bound $\|\quadErr{t}\|$ as 
    \begin{align*}
        \|\quadErr{t}\|
        &\le 2 \rho \escRad \cdot c \escIter \beta_t \step \Delta \sqrt{\logErr} \\
        &= 2 c \crad \cit \beta_t \Delta \sqrt{\logErr},
    \end{align*}
    where the last equality is due to our choice of parameters in \Cref{def:params}:
    \[
        \escRad \escIter
        = \crad \sqrt {\alpha / \rho} \cdot \cit \frac {1} {\step \sqrtra}
        = \frac{\crad \cit}{\rho \step}
    \]

    \paragraph{Bounding $\sgdErr{t}$}
    
    % To bound $\sgdErr{t}$, we use that $\difsgdNoise{t}$ is $\mathrm{nSG}(\sigma)$:
    % \begin{align*}
    %     \|\difsgdNoise{t}\|
    %     = \|\nabla f_{\batch{t}}(\x{t}) - \nabla f_{\batch{t}}(\tx{t})\|
    %     \le L \|\difx{t}\|
    % \end{align*}
    %
    By \Cref{ass:grad_concentration}, each $\sgdErr{t}$ is $\mathrm{nSG}(\sigma^2 / B)$.
    Using the concentration inequality for nSG variables, with probability at least $1 - \tdelta$ we have
    \begin{align*}
        \|\sgdErr{t}\|
        &= \norm{\step \sum_{\tau = 0}^{t - 1} (\id - \step H)^{t - 1 - \tau} \difsgdNoise{\tau}} \\
        &\le \step \sqrt{\sum_{\tau = 0}^{t - 1} (1 + \step \eigen)^{2(t - 1 - \tau)} \frac{\sigma^2}{B}} \cdot \sqrt{\logErr} \\
        &\le \step \sigma \beta_t \sqrt{\logErr} / \sqrt{B} \\
    \end{align*}
    Using assumption $\Delta^2 \ge \sigma^2 / B$, we get the desired bound.
\end{proof}

\begin{lemma}
    \label{lem:bucket_change}
    When $\Delta^2 \ge \sigma^2 / B$, with probability at least $1 - \tdelta$, we have
    \[
        f(\x{0}) - f(\x{\escIter}) > -\df / 100
    \]
    Moreover, with probability at least $1/3 - \tdelta$, we have:
    \[
        f(\x{0}) - f(\x{\escIter}) > \df
    \]
\end{lemma}

\begin{proof}
    The first claim follows from the descent lemma by our choice of parameters:
    \[
        f(\x{0}) - f(\x{\escIter})
        > -c \step \fullVar^2 (\step L \escIter + \logErr)
        > -\df / 10
    \]
    From Corollary~\ref{cor:i_or_l}, we know that with probability at least $1-\tdelta$, if $\|\x{t} - \x{0}\| > \escRad$ for some $t \le \escIter$, then $f(\x{0}) - f(\x{t}) > \df$ with probability at least $1 - \tdelta$.
    Since the $\tx{t}$ has the same distribution as $\x{t}$, the same holds for $\|\tx{t} - \x{0}\|$.
    Hence, if either $\|\x{t} - \x{0}\| > \escRad$ or $\|\tx{t} - \x{0}\| > \escRad$, then with probability $\frac{1}{2} - 2 \tdelta$ we have $f(\x{0}) - f(\x{t})$.
    
    For the rest of the proof, we can assume that $\|\x{t} - \x{0}\| < \escRad$ and $\|\tx{t} - \x{0}\| < \escRad$ for all $t \le \escIter$.
    By Lemmas~\ref{lem:good_term} and~\ref{lem:error_terms} we know that $\|\dif{\escIter}\| \ge \step \beta_t \Delta \sqrt{\logErr} / 10$ and $\|\sgdErr{t} + \quadErr{t}\| \le \step \beta_t \Delta \sqrt{\logErr} / 20$ with probability $1 - \tdelta$.
    Hence,
    \begin{align*}
        \max(\|\x{\escIter} - \x{0}\|, \|\tx{\escIter} - \x{0}\|)
        &\ge \frac{1}{2} \|\difx{\escIter}\| \\
        &\ge \frac 12 \pars{\|\dif{\escIter}\| - \|\sgdErr{\escIter} + \quadErr{t}\|} \\
        &\ge \frac{\step \beta_\escIter \Delta}{40} \sqrt{\logErr} \\
        &= (1 + \step \eigen)^\escIter \frac{1}{40}  \Delta \sqrt{\frac{\step}{\eigen}} \sqrt{\logErr} \\
        &\ge \escRad,
    \end{align*}
    where the last inequality follows by the appropriate choice of logarithmic term in $\cit$ (note that $(1 + \step \eigen)^\escIter$ dominates other terms).
    This contradicts the assumption $\max(\|\x{\escIter} - \x{0}\|, \|\tx{\escIter} - \x{0}\|) \le \escRad$.
\end{proof}

\begin{lemma}
    \label{lem:quarter_saddle}
    When $\Delta^2 \ge \sigma^2 / B$, for $T = 64 \fmax / (\step \alpha^2)$, with $\step$ chosen as in \Cref{def:params}, with probability at least $1 - \tdelta$ we have $\lmin(\nabla^2 f(\x{t})) < -\sqrtra$ for at most $T/4$ points $\x{t}$.
\end{lemma}

\begin{proof}
    \todo{Error probability}
    Proof by contradiction.
    Let's split all iterations $0,...,T-1$ into buckets of size $\escIter$.
    There are $T/\escIter = 64\fmax \sqrtra / \cit$ buckets, and at least quarter of the buckets have a point $\x{t}$ with $\lmin(\nabla^2 f(\x{t})) < -\sqrtra$ in it.
    Note that within each bucket, by Lemma~\ref{lem:bucket_change}, the objective increases by at most $\df / 100$.
    Out of such buckets, at least half of them are non-adjacent, and we consider points $\x{t}$ with $\lmin(\nabla^2 f(\x{t})) < -\sqrtra$ in these buckets.
    With probability at least $1/3 - \tdelta$, we have $f(\x{t}) - f(\x{t + \escIter}) > \df$ for each such $\x{t}$.
    % \todo[inline]{Properly handle logs}
    Hence,
    \begin{align*}
        \fmax
        &\ge \frac{T \df}{10\cdot \escIter} \\
        &= \frac{1}{10} \cdot \frac{64\fmax}{\step \alpha^2} \cdot \cf \sqrtfacr \cdot \frac{\step \sqrtra}{\cit} \\
        &= \fmax \frac{64 \cdot \cf}{10 \cdot \cit}
    \end{align*}
    Hence, by selecting $\cit$ and $\cf$ so that $\frac{64 \cdot \cf}{10 \cdot \cit} > 1$, we arrive at contradiction.
\end{proof}

        % \begin{aligned}
        %     \text{Step size} && \step &= \cstep \frac{1}{L (1 + \tsigma^2)} \\
        %     \text{Total number of iterations} && T &= \frac{64\fmax}{\step \alpha^2} \\
        %     \text{Iterations required for escaping} && \escIter &=  \cit \frac {1} {\step \sqrtra} \\
        %     \text{Escaping radius} && \escRad &= \crad \sqrt {\frac {\alpha} \rho} \\
        %     \text{Objective decrease after successful escaping} && \df &= \cf \sqrtfacr
        %     % \text{Noise standard deviation} && r &= \cnoise \frac \alpha {\sqrt{\gradLip \step}}
        % \end{aligned}\label{eq:params}


% \begin{theorem}[Large-gradient case]
%     If $\|\|$
% \end{theorem}

\begin{theorem}
    \label{thm:combine}
    When $\Delta^2 \ge \sigma^2 / B$, for $T = 64 \fmax / (\step \alpha^2)$, with probability at least $1 - \tdelta$, at least half of visited points are $\alpha$-SOSP.
\end{theorem}
\begin{proof}
    From Lemma~\ref{lem:quarter_large_grad}, we know that the number of points with large gradient is at most $T/4$.
    From Lemma~\ref{lem:quarter_saddle} we know that the number of points $\x{t}$ with $\lmin(\nabla^2 f(\x{t})) < -\sqrtra$ is at most $T/4$.
    Hence, at least half of the points are $\alpha$-SOSP.
\end{proof}



==> v1_proof_convergence.tex <==
\section{Convergence Proof}

\begin{assumption}
    \label{ass:main_new}
    The objective function $f$ and the component functions $f_i$ satisfy the following conditions.
    \begin{enumerate}
        {\color{green}\item (Boundedness) 
            There exists $\fmax$ such that $\fmax > f(\x{0}) - f(\vx^*)$.}
        {\color{green}\item (Smoothness) $f$ is $L$-smooth, i.e. $\norm{\nabla f(\vx) - \nabla f(\vy)} \le L \norm{\vx - \vy}$ for all $\vx, \vy \in \R^d$.\todo{Check that we cak reuse the gradient norm bound}}
        {\color{green}\item (Lipschitz Hessian) The objective function $f$ has a $\rho$-Lipschitz Hessian, i.e. $\norm{\nabla^2 f(\vx) - \nabla^2 f(\vy)} \le \rho \norm{\vx - \vy}$ for all $\vx, \vy \in \R^d$.}
        {\color{red}\item (Relaxed Stochastic variance) The stochastic variance is bounded as follows: $\avg_{i=1}^N \norm{\nabla f_i(\vx) - \nabla f(\vx)}^2 \le \sigma_1^2 \SqrNorm{\nabla f(\vx)} + \sigma_2^2$.}
    \end{enumerate}
\end{assumption}

\todo{Rewrite}
\begin{assumption}
    {\color{red}No nSG assumption.}
\end{assumption}
\begin{assumption}
    {\color{red}Clipping. (Not doable quickly)}
\end{assumption}

\label{app:convergence_proof}

\todo{Mention that mostly follows Jin et al.}

\begin{definition}
    \label{def:params}
    Let $\fullVar = \nicefrac{\sigma^2}{B} + d \Delta^2$ be total noise variance.
    Our choice of parameters is the following ($\cstep, \cit, \crad, \cf$ hide polylogarithmic dependence on all parameters):
    \begin{equation*}
        \begin{aligned}
            \text{Step size} && \step &= \cstep \min\pars{\frac{\alpha^2}{L (1 + \tsigma^2)}, \frac{\fmax}{L \tsigma^2}} \\
            \text{Total number of iterations} && T &= \frac{64\fmax}{\step \alpha^2} \\
            \text{Iterations required for escaping} && \escIter &=  \cit \frac {1} {\step \sqrtra} \\
            \text{Escaping radius} && \escRad &= \crad \sqrt {\alpha / \rho} \\
            \text{Objective decrease after successful escaping} && \df &= \cf \sqrtfacr
            % \text{Noise standard deviation} && r &= \cnoise \frac \alpha {\sqrt{\gradLip \step}}
        \end{aligned}
        % \label{eq:params}
    \end{equation*}
\end{definition}
Intuitively, the parameters are chosen as follows.
Assume that the current point is $\vzero$ and the function is quadratic, i.e. $f(\vx) = \vx^T H \vx$.
If $\vx$ is a saddle point, then we know that the smallest eigenvalue of $H$ is $-\eigen < -\sqrtra$ with the corresponding eigenvector $\vv_1$.
Then, the largest function decrease would be in the direction of $\vv_1$, and this direction can be found using power method for the appropriate matrix.
But, if we look at the gradient descent update:
\[
    \x{t+1}
    = \x{t} - \step \nabla f(\x{t})
    = \x{t} - \step 2 H \x{t}
    = (\id - \step 2 H) \x{t},
\]
we see that for quadratic functions, gradient descent is exactly the power method for the matrix $\id - \step 2H$, which has the same eigenvectors as $H$. The eigenvalue $-\eigen$ of $H$ corresponds to the eigenvalue $1 + 2 \step \eigen$ of $1 - \step 2 H$, which is the largest (by absolute value) eigenvalue when $\step \le 1/L$.
Note that power method requires some initial randomness, which explains while randomness is required to escape from saddle points.

The above intuition motivates the choice of parameters.
\begin{itemize}
    \item
        \textbf{Escaping radius $\escRad$}. Since in general the function is not necessarily quadratic, we want to guarantee that the Hessian doesn't change excessively.
        More specifically, we want the smallest eigenvalue to be at most $-\eigen / 2$ for the entire escaping procedure.
        By the Hessian-Lipschitz property $\|\nabla^2 f(\vx) - \nabla^2 f(\vy)\| \le \rho \|\vx - \vy\|$, if we work in the radius $\escRad = \eigen /(2\rho)$, then for any point within the radius $\escRad$ of the initial point, the smallest eigenvalue is at most $-\eigen + \eigen / 2 = -\eigen / 2$.
        When $\eigen > \sqrtra$, we can lower-bound $\escRad$ as $\sqrtra / (2\rho) = \sqrt{\alpha / (4\rho)}$.
    \item
        \textbf{Number of iterations required for escaping $\escIter$}.
        After $t$ iterations, the length of $\x{t}$ along the $\vv_1$ direction is $(1 + \step \eigen)^t \approx e^{t / (\step \eigen)}$.
        Hence, we reach the boundary of the ball of radius $\escRad$ after $(t \log \escRad) / (\step \eigen)$ iterations.
    \item
        \textbf{Function change after escaping $\df$}.
        Since we are working inside the ball of size $\escRad$, the best objective improvement $\df$ we can aim for is achievable by moving by $\escRad \vv_1$.
        This improves the objective by approximately $\escRad^2 \eigen$, which, by the choice of the parameters can be lower-bounded as $\alpha / \rho \cdot \sqrtra = \sqrt{\alpha^3 / \rho}$.
    \item
        \textbf{Total number of iterations $T$}. Every $\escIter$ iterations we improve objective by $\df$.
        Since the total objective improvement cannot exceed $\fmax$, the maximum number of iterations is
        \[
            \frac{\fmax \escIter}{\df}
            \le \frac{\fmax}{(\step \sqrtra)\sqrt{\alpha^3 / \rho}}
            = \frac{\fmax}{\step \alpha^2}
        \]
\end{itemize}

\begin{lemma}[Descent Lemma]
    \label{lem:descent}
    Assume that $\step < 1/L$, for any $t_0$ and $t$.
    Then, with probability at least $1 - \tdelta$, for some constant $c$:
    \[
        f(\x{t_0}) - f(\x{t_0 + t})
        \ge \frac{\step}{8} \sum_{\tau=t_0}^{t_0 + t - 1} \norm{\nabla f(\x{\tau})}^2 - c \step \tsigma^2 (\step L t + \logErr)
        .
    \]
\end{lemma}

\begin{proof}
    W.l.o.g., we consider $t_0 = 0$.
    Let $\sgdNoise{\tau} = \nabla f_{\batch{t}}(\x{\tau}) - \nabla f(\x{\tau})$ be the stochastic noise at iteration $\tau$.
    By the folklore Descent Lemma,
    \begin{align*}
        f(\x{\tau}) - f(\x{\tau+1})
        % \ge \step \sum_{\tau=0}^{t-1} \InnerProd{\nabla f(\x{\tau}), \nabla f_{\batch{t}}(\x{\tau})}
            % - \frac{L}{2} \SqrNorm{\x{}}
        &\ge \step \InnerProd{\nabla f(\x{\tau}), \nabla f_{\batch{t}}(\x{\tau})}
            - \frac{L}{2} \SqrNorm{\x{\tau + 1} - \x{\tau}} \\
        &= \step \InnerProd{\nabla f(\x{\tau}), \nabla f(\x{\tau}) + \sgdNoise{\tau} + \ourNoise{\tau}}
            - \frac{L\step^2}{2} \SqrNorm{\nabla f(\x{\tau}) + \sgdNoise{\tau} + \ourNoise{\tau}} \\
        &\ge \step \SqrNorm{\nabla f(\x{\tau})} + \step \InnerProd{\nabla f(\x{\tau}), \sgdNoise{\tau} + \ourNoise{\tau}}
            - \frac{\step^2 L}{2} \pars{\frac{3}{2}\SqrNorm{\nabla f(\x{\tau})} + 3 \SqrNorm{\sgdNoise{\tau} + \ourNoise{\tau}}}
        % &= \step \InnerProd{\nabla f(\x{\tau}), \nabla f(\x{\tau}) + \sgdNoise{\tau}}
        %     - \frac{L\step^2}{2} \SqrNorm{\nabla f(\x{\tau}) + \sgdNoise{\tau}} \\
        ,
    \end{align*}
    where we used inequality $\|a + b\|^2 \le (1 + \nu) \|a\|^2 + (1 + 1/\nu)\|b\|^2$ for $\nu = 1/2$.
    By telescoping, we have:
    \begin{align*}
        f(\x{0}) - f(\x{t})
        &\ge \frac{\step}{4} \sum_{\tau=0}^{t-1} \SqrNorm{\nabla f(\x{\tau})} + \step \sum_{\tau=0}^{t-1} \InnerProd{\nabla f(\x{\tau}), \sgdNoise{\tau} + \ourNoise{\tau}}
            - \frac{3 \step^2 L}{2} \sum_{\tau=0}^{t-1} \SqrNorm{\sgdNoise{\tau} + \ourNoise{\tau}}
        % &= \step \InnerProd{\nabla f(\x{\tau}), \nabla f(\x{\tau}) + \sgdNoise{\tau}}
        %     - \frac{L\step^2}{2} \SqrNorm{\nabla f(\x{\tau}) + \sgdNoise{\tau}} \\
    \end{align*}
    %
    Using a concentration inequality for nSG variables, with probability at least $1 - \tdelta$ for some constant $c$ we have
    \[
        \abs{\step \sum_{\tau=0}^{t-1} \InnerProd{\nabla f(\x{\tau}), \sgdNoise{\tau} + \ourNoise{\tau}}}
        \le \frac{\step}{8} \sum_{\tau=0}^{t-1} \SqrNorm{\nabla f(\x{\tau})} + c \step \fullVar^2 \logErr
    \]
    \todo{Give reference}
    \todo{Avoid norm-subGaussian}
    For the last term, with probability at least $1 - \tdelta$ we have
    \[
        \frac{3 \step^2 L}{2} \sum_{\tau=0}^{t-1} \SqrNorm{\sgdNoise{\tau}}
        \le c \step^2 L \fullVar^2 (t + \logErr).
    \]
    Combining the above inequalities and using $\step \le 1/L$ finishes the proof.
    % \todo{TODO}
\end{proof}

\subsection{Large Gradient Case}

The first application of the Descent Lemma is to bound the number of iterations when the gradient is large.
\begin{lemma}
    \label{lem:quarter_large_grad}
    When $T \ge \frac{64 \fmax}{\step \alpha^2}$ and other parameters are as in \Cref{def:params}, the number of iterations $t$ with $\|\nabla f(\x{t})\| \ge \alpha$ is at most $\nicefrac T4$.
\end{lemma}

\begin{proof}
    For the sake of contradiction, assume that the number of points $\x{t}$ with $\|\nabla f(\x{t})\| \ge \alpha$ is greater than $\nicefrac T4$.
    Then, by the Descent Lemma we have
    \begin{align*}
        f(\x{0}) - f(\x{T})
        &\ge \frac{\step}{8} \sum_{\tau=0}^{T - 1} \norm{\nabla f(\x{\tau})}^2 - c \step \tsigma^2 (\step L T + \logErr) \\
        &\ge \frac{\step T \alpha^2}{32}  - c \step T \cdot \tsigma^2 \pars{\step L + \frac{\logErr}{T}}
    \end{align*}
    We will show that the right-hand side is at least $\fmax$, leading to contradiction.
    For that, it suffices to guarantee that $\frac{\step T \alpha^2}{32} \ge 2\fmax$ and $c \step T \cdot \tsigma^2 \pars{\step L + \frac{\logErr}{T}} \le \fmax$.
    The former condition is satisfied by our choice of $T$, and substituting the bound on $\fmax$ into the latter condition shows that it suffices to prove
    \[
        64 c \tsigma^2 \pars{\step L + \frac{\step \alpha^2 \logErr}{64 \fmax}} \le \alpha^2
    \]
    It suffices to bound each term with $\alpha^2 / 2$, which is satisfied for
    \begin{align*}
        \step &\le \frac{\alpha^2}{128 \cdot c \tsigma^2 L} \\
        \step &\le \frac{\fmax\logErr}{2 \cdot c \tsigma^2 L}
    \end{align*}
    Both of these conditions are satisfied by our choice of $\step$, with the appropriate choice of $\cstep$.
\end{proof}




\subsection{Escaping From Saddle Points}

The Descent Lemma also implies the following result, which upper-bounds the distance change in terms of the objective changes.
Its \Cref{cor:i_or_l} states that, if after a bounded number of iterations the point moves far from the original point, then the objective value sufficiently decreases.
%
\begin{lemma}[Improve or localize]
    \label{lem:improve_or_localize}
    For any $t_0$ and $t$, with probability at least $1 - \tdelta$, for some constant $c$:
    \begin{align*}
        \SqrNorm{\x{t_0 + t} - \x{t_0}}
        \le c \step t \pars{(f(\x{t_0}) - f(\x{t_0 + t}) + \step \tsigma^2 (\step L t + \logErr)}
    \end{align*}
\end{lemma}
%
\begin{proof}
    W.l.o.g. we consider the case when $t_0 = 0$.
    % By the Descent Lemma,
    % \[
    %     f(\x{0}) - f(\x{t})
    %     \ge \frac{\step}{8} \sum_{\tau=0}^{t - 1} \norm{\nabla f(\x{\tau})}^2 - c \step \tsigma^2 (\step L t + \logErr)
    % \]
    By the definition of $\x{\tau + 1}$, we have
    \begin{align*}
        \x{\tau} - \x{\tau + 1}
        = \step (\nabla f_{\batch{\tau}}(\x{\tau}) + \ourNoise{\tau})
        = \step (\nabla f(\x{\tau}) + \sgdNoise{\tau} + \ourNoise{\tau}),
    \end{align*}
    where $\sgdNoise{\tau} = \nabla f_{\batch{\tau}}(\x{\tau}) - \nabla f(\x{\tau})$ is stochastic gradient noise.
    By telescoping, we have:
    \begin{align*}
        \|\x{0} - \x{t}\|
        &= \step \norm{\sum_{\tau = 0}^{t - 1}(\nabla f(\x{\tau}) + \sgdNoise{\tau} + \ourNoise{\tau})}
    \end{align*}
    By Cauchy-Schwarz Inequality, we have:
    \begin{align*}
        \|\x{0} - \x{t}\|^2
        &\le 2 \step^2 \pars{\norm{\sum_{\tau = 0}^{t - 1}\nabla f(\x{\tau})}^2 + \norm{\sum_{\tau = 0}^{t - 1} (\sgdNoise{\tau} + \ourNoise{\tau})}^2} \\
        &\le 2 \step^2 \pars{t \sum_{\tau = 0}^{t - 1}\norm{\nabla f(\x{\tau})}^2 + \norm{\sum_{\tau = 0}^{t - 1} (\sgdNoise{\tau} + \ourNoise{\tau})}^2}
    \end{align*}
    \todo{Elaborate and avoid nSG}
    Since $\sgdNoise{\tau} + \ourNoise{\tau}$ is $\mathrm{nSG}(\fullVar^2)$, by applying concentration inequality for $\mathrm{nSG}$ variables, we have with probability at least $1 - \tdelta$:
    \begin{align*}
        \|\x{0} - \x{t}\|^2
        &\le 2 \step^2 \pars{t \sum_{\tau = 0}^{t - 1}\norm{\nabla f(\x{\tau})}^2 + c t \fullVar^2 \logErr}
    \end{align*}
    Finally, applying the Descent Lemma, we get
    \begin{align*}
        \|\x{0} - \x{t}\|^2
        &\le \step c t \pars{f(\x{0}) - f(\x{t}) + \step \fullVar^2 (\step L t + \logErr)}
    \end{align*}
    for some constant $c$.
\end{proof}


\begin{corollary}
    \label{cor:i_or_l}
    For the parameters chosen as in \Cref{def:params}, if for some $t \le \escIter$ we have $\SqrNorm{\x{t_0 + \tau} - \x{t_0}} \ge \escRad$, then $f(\x{t_0}) - f(\x{t_0 + \tau}) \ge \df$ with probability at least $1 - \tdelta$.
\end{corollary}
%
\begin{proof}
    From \Cref{lem:improve_or_localize}, we know that for some $c$:
    \begin{align*}
        f(\x{t_0}) - f(\x{t_0 + t})
        &\ge \frac{\escRad^2}{c \step \escIter} - \step \tsigma^2 (\step L \escIter + \logErr) \\
        &\ge \frac{\crad^2}{c \cit} \sqrtfacr - \step \tsigma^2 \pars{\frac{\cit L}{\sqrtra} + \logErr}
        % &\ge \frac{\SqrNorm{\x{t_0 + t} - \x{t_0}}}{c \step \escIter} - \step \tsigma^2 (\step L \escIter + \log 1/\fullVar)
    \end{align*}
    We want to guarantee that the right-hand side is at most $\df = \cf \sqrtfacr$.
    It suffices to guarantee that
    \begin{align*}
        \crad^2 / (c \cit) \ge 2 \cf \qquad \text{and} \qquad \step \tsigma^2 (\cit L / \sqrtra + \logErr) \le \cf \sqrtfacr.
    \end{align*}
    The former holds for the appropriate choice of $\crad$, $\cit$, and $\cf$, and the latter holds by choosing
    \[
        \step \le (\alpha^2 / L \tsigma^2) \cdot  \cf / \pars{\cit + \logErr},
    \]
    where we assumed $L \ge \sqrtra$, since otherwise any $\alpha$-FOSP is an $\alpha$-SOSP because $L$ is an upper bound on the absolute values of the Hessian.
\end{proof}

\begin{definition}[Coupling sequences]
    \label{def:coupling_sequence}
    Let $\vv_1$ be the eigenvector corresponding to the smallest eigenvalue of $\nabla^2 f(\x{t_0})$.
    The coupling sequences starting from $\x{t_0}$ are defined as follows:
    \begin{equation}
        \begin{aligned}
            \ourNoise{t_0+t} &\sim \mathcal{N}(0, \fullVar^2 \id) \\
                \tourNoise{t_0+t} &= \ourNoise{t_0+t} - 2 \InnerProd{ \vv_1, \ourNoise{t_0+t} } \vv_1  \\
                % \batch'_{t_0+t} &= \batch_{t_0+t}, \\
            \x{t_0 + t+1} &= \x{t_0+t} - \step (\nabla f_{\batch{t}}(\x{t_0 + t}) + \ourNoise{t_0 + t}) \\
            \tx{t_0 + t+1} &= \tx{t_0+t} - \step (\nabla f_{\batch{t}}(\tx{t_0 + t}) + \tourNoise{t_0 + t}) \\
            \sgdNoise{t_0 + t} &= \nabla f_{\batch{t}}(\x{t_0 + t}) - \nabla f(\x{t_0 + t}) \\
            \tsgdNoise{t_0 + t} &= \nabla f_{\batch{t}}(\tx{t_0 + t}) - \nabla f(\tx{t_0 + t}) \\
        \end{aligned}\nonumber
    \end{equation}
    %
    Note that:
    \begin{itemize}
        \item the artificial noise $\tourNoise{t_0 + t}$ has the opposite sign in direction $\vv_1$ compared with $\ourNoise{t_0 + t}$,
        \item the stochastic randomness ${\batch{t}}$ is the same for both sequences,\todo{Might be not required, but anyways makes things simpler to define}
        \item $\{\x{t_0 + t}\}_t$ and $\{\tx{t_0 + t}\}_t$ are sampled from the same distribution.
    \end{itemize}
    %
    We next define the difference between the coupling sequences:
    \begin{equation}
        \begin{aligned}
            \difourNoise{t} &= \xi_{t_0+t} - \xi'_{t_0+t} 
                = 2 \InnerProd{ \vv_1, \xi_{t_0+t} } \vv_1  \\
                % \batch'_{t_0+t} &= \batch_{t_0+t}, \\
            \difx{t_0 + t+1} &= \x{t_0+t} - \tx{t_0+t} \\
            \difsgdNoise{t_0 + t} &= \sgdNoise{t_0 + t} - \tsgdNoise{t_0 + t}
        \end{aligned}\nonumber
    \end{equation}
\end{definition}

% TODO (the rest is standard)

% SGD with variance $\sigma^2$ and batch size $B$, then the number of iterations to find an $\alpha$-FOSP ($\|\nabla f(\vx)\| < \alpha$) is $\frac{\sigma^2}{B \alpha^4}$.

From now on, we assume that we want to escape from point $\x{t_0}$ such that $\lmin(\nabla^2 f(\x{t_0})) < -\sqrtra$.
W.l.o.g. we assume $t_0 = 0$.
Let $H = \nabla^2 f(\x{0})$ be the Hessian of $f$ at point $\x{0}$, let $-\eigen = \lmin(H)$ be the smallest eigenvalue of $H$, and $\vv_1$ be the eigenvector corresponding to $-\eigen$.

\begin{lemma}
    For every $t$,
    \[
        \difx{t} = -\dif{t} - \sgdErr{t} -\quadErr{t},
    \]
    where
    \begin{align*}
        \dif{t} &= \step \sum_{\tau = 0}^{t - 1} (\id - \step H)^{t - 1 - \tau} \difourNoise{\tau} \\
        \sgdErr{t} &= \step \sum_{\tau = 0}^{t - 1} (\id - \step H)^{t - 1 - \tau} \difsgdNoise{\tau} \\
        \quadErr{t} &= \step \sum_{\tau = 0}^{t - 1} (\id - \step H)^{t - 1 - \tau} \hesInt{\tau} \difx{\tau},
            \quad \text{ where } \quad \hesInt{\tau} = \int_0^1  (\nabla^2 f(\psi \x{\tau} + (1 - \psi) \tx{\tau}) - H)\ d\psi
    \end{align*}
\end{lemma}
\begin{proof}
    Proof by induction.
    \begin{align*}
        \difx{t + 1}
        &= \difx{t} - \step (\difsgdNoise{t} + \difsgdNoise{t}) - \step (\nabla f(\x{t}) - \nabla f(\tx{t})) \\
        &= (1 - \step H) \difx{t} - \step (\difsgdNoise{t} + \difsgdNoise{t}) - \step (\nabla f(\x{t}) - \nabla f(\tx{t}) - H \difx{t})
    \end{align*}
    Using that $\nabla f(\x{t}) - \nabla f(\tx{t}) = \int_0^1  \nabla^2 f(\psi \x{\tau} + (1 - \psi) \tx{\tau}) \difx{\tau}\ d\psi$, by telescoping we complete the proof.
\end{proof}
%
In the following statements, the geometric series $\alpha_t^2 = \sum_{\tau = 0}^{t-1} (1 + \step \eigen)^{2 \tau}$ occurs frequently.
Intuitively, each iteration increases the distance approximately by a factor of $(1 + \step \eigen)$~-- the largest eigenvalue of matrix $I - \step H$.
The noise added at iteration $\tau$ gets amplified by $(1 + \step \eigen)^{t - \tau}$ by iteration $t$, and, if every iteration an independent noise of variance $\Delta^2$ is added, $\Delta^2 \alpha_t^2$ is the total variance of such a noise accumulated over the iterations.
%
\begin{lemma}
    \label{lem:alpha_beta}
    Let $\alpha_t = \sqrt{\sum_{\tau = 0}^{t-1} (1 + \step \eigen)^{2 \tau}}$ and $\beta_t = (1 + \step \eigen)^t / \sqrt{\step \eigen}$.
    If $\step \eigen < 1$, then $\alpha_t \le \beta_t$ for any $t$ and $\alpha_t \ge \beta_t / 3$ for $t \ge 2 / (\step \eigen)$.
\end{lemma}
\begin{proof}
    As a sum of geometric progression, we have
    \[
        \alpha_t^2
        = \frac{(1 + \step \eigen)^{2t} - 1}{(1 + \step \eigen)^2 - 1}
        = \frac{(1 + \step \eigen)^{2t} - 1}{\step \eigen (2 + \step \eigen)},
    \]
    and $\alpha_t^2 \le \beta_t^2$ follows immediately.
    On the other hand, for $t \ge 1 / (\step \eigen)$ we have $(1 + \step \eigen)^{2t} \ge 2$, and hence $(1 + \step \eigen)^{2t}  - 1 \ge (1 + \step \eigen)^{2t} / 2$.
    Finally, by our choice of the step size, we have $\step \eigen \le \step L \le 1$, and hence $2 + \step \eigen \le 3$.
    This implies $\alpha_t^2 \ge \beta_t^2 / 6$, finishing the proof.
\end{proof}

\begin{lemma}
    \label{lem:good_term}
    Let $\beta_t = (1 + \step \eigen)^t / \sqrt{\step \eigen}$.
    Then for any $t$ and $\tdelta$, for some constant $c$:
    \begin{align*}
        \P{\|\dif{t}\| \ge c \beta_t \step \Delta \sqrt{\logErr}} &\le \tdelta \\
        \P{\|\dif{t}\| \le \frac{\beta_t \step \Delta}{10}} &\le \frac 13
    \end{align*}
\end{lemma}
\todo{Check $\sqrt{\logErr}$}

\begin{proof}
    Since $\difourNoise{\tau} = 2\InnerProd{\ourNoise{\tau}, \vv_1} \vv_1$ and $\vv_1$ is an eigenvalue of $H$ corresponding to eigenvalue $-\eigen$, we have
    \[
        \dif{t}
        = \step \sum_{\tau = 0}^{t - 1} (\id - \step H)^{t - 1 - \tau} \difourNoise{\tau}
        = \pars{\step \sum_{\tau = 0}^{t - 1} (1 + \step \eigen)^{t - 1 - \tau} \InnerProd{\ourNoise{\tau}, \vv_1}} \vv_1
    \]
    Hence, $\dif{t}$ is a random variable which is parallel to $\vv_1$.
    % Hence, $\dif{t}$ is a Gaussian random variable along direction $\vv_1$ with variance $\step \sum_{\tau = 0}^{t - 1} (1 + \step \eigen)^{t - 1 - \tau} \InnerProd{\ourNoise{\tau}, \vv_1}$
    Since each $\ourNoise{t}$ is a Gaussian random variable with the covariance matrix $\Delta^2 \id$, each $\InnerProd{\ourNoise{t}, \vv_1}$ a Gaussian random variable with variance $\Delta^2$.
    Hence, $\dif{t}$ is also a Gaussian random variable, and
    \[
        \Var{\|\dif{t}\|}
        = \step \sum_{\tau = 0}^{t - 1} (1 + \step \eigen)^{\tau} \Delta^2
        = \Delta^2 \alpha_t^2
    \]
    The upper bound on $\|\dif{t}\|$ follows from \Cref{lem:alpha_beta} and standard concentration inequality for Guassians.
    The lower bound follows from inequality $\P{|X| \le \sigma a} \le a$ for $X \sim \mathcal{N}(0, \sigma^2)$ and any $a$.
\end{proof}

\todo{Be more careful with $\tdelta$}

\todo{Replace $\fullVar$ with $\Delta$ where required}

\todo{Propagate assumption $\Delta^2 \ge \sigma^2 / B$}

\begin{lemma}
    \label{lem:error_terms}
    Let $\mathcal{E}_t$ be the event ``$\|\x{0} - \x{\tau}\| < \escRad$ and $\|\x{0} - \tx{\tau}\| < \escRad$ for all $\tau < t$''.
    Then, when $\Delta^2 \ge \sigma^2 / B$, for some constant $c$ we have
    % \todo[inline]{Fix log error}
    \[
        \P{\mathcal{E}_\escIter
            \implies \max\nolimits_{\tau=0}^{\escIter - 1} \norm{\sgdErr{\tau} + \quadErr{\tau}}
            \le 
            c \beta_\tau \step \Delta \sqrt{\logErr}
        } \ge 1 - \escIter \tdelta
    \]
\end{lemma}
    
\begin{proof}
    By induction on $t$, we will prove that $\P{\mathcal{E}_t \implies \|\difx{t}\| \le c \step \Delta \beta_t} \le 1 - t\fullVar$ and
    \[
        \P{\mathcal{E}_t
            \implies \max\nolimits_{\tau=0}^{t - 1} \norm{\sgdErr{\tau} + \quadErr{\tau}}
            \le  c \beta_\tau \step \Delta \sqrt{\logErr}
        } \ge 1 - t \tdelta.
    \]
    Base case is $t=0$, in which case $\difx{0} = \vzero$.
    For the induction step, since $\difx{t} = -\dif{t} - \sgdErr{t} -\quadErr{t}$, we bound each term separately.
    \paragraph{Bounding $\dif{t}$}
    By \Cref{lem:good_term}, we have $\P{\|\dif{t}\| \ge c \beta_t \step \Delta \sqrt{\logErr}} \le \tdelta$.

    
    \paragraph{Bounding $\quadErr{t}$}
    Assuming $\mathcal{E}_t$, by the Hessian-Lipschitz property we have
    \begin{align*}
        \|\hesInt{\tau} \difx{\tau}\|
        &= \norm{\int_0^1  (\nabla^2 f(\psi \x{\tau} + (1 - \psi) \tx{\tau}) - H)\ d\psi \cdot \difx{\tau}} \\
        &\le 2 \rho \escRad \|\difx{\tau}\| \\
        &\le 2 \rho \escRad \cdot c \beta_\tau \step \Delta \sqrt{\logErr},
    \end{align*}
    %
    and we bound $\quadErr{t}$ as
    %
    \begin{align*}
        \|\quadErr{t}\|
        &= \norm{\step \sum_{\tau = 0}^{t - 1} (\id - \step H)^{t - 1 - \tau} \hesInt{\tau} \difx{\tau}} \\
        &\le \sum_{\tau = 0}^{t - 1} (1 + \step \gamma)^{t - 1 - \tau} 2 \rho \escRad \cdot c \beta_\tau \step \Delta \sqrt{\logErr} \\
        % &\le \sum_{\tau = 0}^{t - 1} (1 + \step \gamma)^{\tau} 2 \rho \escRad \cdot c \beta_t \step \fullVar^2 \sqrt{\logErr} \\
    \end{align*}
    Since $(1 + \step \gamma)^{t - 1 - \tau} \beta_\tau = \beta_{t-1}$,
    % \[
    %     \sum_{\tau = 0}^{t - 1} (1 + \step \gamma)^{\tau}
    %     = \frac{(1 + \step \gamma)^t - 1}{\step \gamma}
    %     \le \frac{\beta_t}{\sqrt{\step \gamma}},
    % \]
    we can bound $\|\quadErr{t}\|$ as 
    \begin{align*}
        \|\quadErr{t}\|
        &\le 2 \rho \escRad \cdot c \escIter \beta_t \step \Delta \sqrt{\logErr} \\
        &= 2 c \crad \cit \beta_t \Delta \sqrt{\logErr},
    \end{align*}
    where the last equality is due to our choice of parameters in \Cref{def:params}:
    \[
        \escRad \escIter
        = \crad \sqrt {\alpha / \rho} \cdot \cit \frac {1} {\step \sqrtra}
        = \frac{\crad \cit}{\rho \step}
    \]

    \paragraph{Bounding $\sgdErr{t}$}
    
    % To bound $\sgdErr{t}$, we use that $\difsgdNoise{t}$ is $\mathrm{nSG}(\sigma)$:
    % \begin{align*}
    %     \|\difsgdNoise{t}\|
    %     = \|\nabla f_{\batch{t}}(\x{t}) - \nabla f_{\batch{t}}(\tx{t})\|
    %     \le L \|\difx{t}\|
    % \end{align*}
    %
    By \Cref{ass:grad_concentration}, each $\sgdErr{t}$ is $\mathrm{nSG}(\sigma^2 / B)$.
    Using the concentration inequality for nSG variables, with probability at least $1 - \tdelta$ we have
    \begin{align*}
        \|\sgdErr{t}\|
        &= \norm{\step \sum_{\tau = 0}^{t - 1} (\id - \step H)^{t - 1 - \tau} \difsgdNoise{\tau}} \\
        &\le \step \sqrt{\sum_{\tau = 0}^{t - 1} (1 + \step \eigen)^{2(t - 1 - \tau)} \frac{\sigma^2}{B}} \cdot \sqrt{\logErr} \\
        &\le \step \sigma \beta_t \sqrt{\logErr} / \sqrt{B} \\
    \end{align*}
    Using assumption $\Delta^2 \ge \sigma^2 / B$, we get the desired bound.
\end{proof}

\begin{lemma}
    \label{lem:bucket_change}
    When $\Delta^2 \ge \sigma^2 / B$, with probability at least $1 - \tdelta$, we have
    \[
        f(\x{0}) - f(\x{\escIter}) > -\df / 100
    \]
    Moreover, with probability at least $1/3 - \tdelta$, we have:
    \[
        f(\x{0}) - f(\x{\escIter}) > \df
    \]
\end{lemma}

\begin{proof}
    The first claim follows from the descent lemma by our choice of parameters:
    \[
        f(\x{0}) - f(\x{\escIter})
        > -c \step \fullVar^2 (\step L \escIter + \logErr)
        > -\df / 10
    \]
    From Corollary~\ref{cor:i_or_l}, we know that with probability at least $1-\tdelta$, if $\|\x{t} - \x{0}\| > \escRad$ for some $t \le \escIter$, then $f(\x{0}) - f(\x{t}) > \df$ with probability at least $1 - \tdelta$.
    Since the $\tx{t}$ has the same distribution as $\x{t}$, the same holds for $\|\tx{t} - \x{0}\|$.
    Hence, if either $\|\x{t} - \x{0}\| > \escRad$ or $\|\tx{t} - \x{0}\| > \escRad$, then with probability $\frac{1}{2} - 2 \tdelta$ we have $f(\x{0}) - f(\x{t})$.
    
    For the rest of the proof, we can assume that $\|\x{t} - \x{0}\| < \escRad$ and $\|\tx{t} - \x{0}\| < \escRad$ for all $t \le \escIter$.
    By Lemmas~\ref{lem:good_term} and~\ref{lem:error_terms} we know that $\|\dif{\escIter}\| \ge \step \beta_t \Delta \sqrt{\logErr} / 10$ and $\|\sgdErr{t} + \quadErr{t}\| \le \step \beta_t \Delta \sqrt{\logErr} / 20$ with probability $1 - \tdelta$.
    Hence,
    \begin{align*}
        \max(\|\x{\escIter} - \x{0}\|, \|\tx{\escIter} - \x{0}\|)
        &\ge \frac{1}{2} \|\difx{\escIter}\| \\
        &\ge \frac 12 \pars{\|\dif{\escIter}\| - \|\sgdErr{\escIter} + \quadErr{t}\|} \\
        &\ge \frac{\step \beta_\escIter \Delta}{40} \sqrt{\logErr} \\
        &= (1 + \step \eigen)^\escIter \frac{1}{40}  \Delta \sqrt{\frac{\step}{\eigen}} \sqrt{\logErr} \\
        &\ge \escRad,
    \end{align*}
    where the last inequality follows by the appropriate choice of logarithmic term in $\cit$ (note that $(1 + \step \eigen)^\escIter$ dominates other terms).
    This contradicts the assumption $\max(\|\x{\escIter} - \x{0}\|, \|\tx{\escIter} - \x{0}\|) \le \escRad$.
\end{proof}

\begin{lemma}
    \label{lem:quarter_saddle}
    When $\Delta^2 \ge \sigma^2 / B$, for $T = 64 \fmax / (\step \alpha^2)$, with $\step$ chosen as in \Cref{def:params}, with probability at least $1 - \tdelta$ we have $\lmin(\nabla^2 f(\x{t})) < -\sqrtra$ for at most $T/4$ points $\x{t}$.
\end{lemma}

\begin{proof}
    \todo{Error probability}
    Proof by contradiction.
    Let's split all iterations $0,...,T-1$ into buckets of size $\escIter$.
    There are $T/\escIter = 64\fmax \sqrtra / \cit$ buckets, and at least quarter of the buckets have a point $\x{t}$ with $\lmin(\nabla^2 f(\x{t})) < -\sqrtra$ in it.
    Note that within each bucket, by Lemma~\ref{lem:bucket_change}, the objective increases by at most $\df / 100$.
    Out of such buckets, at least half of them are non-adjacent, and we consider points $\x{t}$ with $\lmin(\nabla^2 f(\x{t})) < -\sqrtra$ in these buckets.
    With probability at least $1/3 - \tdelta$, we have $f(\x{t}) - f(\x{t + \escIter}) > \df$ for each such $\x{t}$.
    % \todo[inline]{Properly handle logs}
    Hence,
    \begin{align*}
        \fmax
        &\ge \frac{T \df}{10\cdot \escIter} \\
        &= \frac{1}{10} \cdot \frac{64\fmax}{\step \alpha^2} \cdot \cf \sqrtfacr \cdot \frac{\step \sqrtra}{\cit} \\
        &= \fmax \frac{64 \cdot \cf}{10 \cdot \cit}
    \end{align*}
    Hence, by selecting $\cit$ and $\cf$ so that $\frac{64 \cdot \cf}{10 \cdot \cit} > 1$, we arrive at contradiction.
\end{proof}

        % \begin{aligned}
        %     \text{Step size} && \step &= \cstep \frac{1}{L (1 + \tsigma^2)} \\
        %     \text{Total number of iterations} && T &= \frac{64\fmax}{\step \alpha^2} \\
        %     \text{Iterations required for escaping} && \escIter &=  \cit \frac {1} {\step \sqrtra} \\
        %     \text{Escaping radius} && \escRad &= \crad \sqrt {\frac {\alpha} \rho} \\
        %     \text{Objective decrease after successful escaping} && \df &= \cf \sqrtfacr
        %     % \text{Noise standard deviation} && r &= \cnoise \frac \alpha {\sqrt{\gradLip \step}}
        % \end{aligned}\label{eq:params}


% \begin{theorem}[Large-gradient case]
%     If $\|\|$
% \end{theorem}

\begin{theorem}
    \label{thm:combine}
    When $\Delta^2 \ge \sigma^2 / B$, for $T = 64 \fmax / (\step \alpha^2)$, with probability at least $1 - \tdelta$, at least half of visited points are $\alpha$-SOSP.
\end{theorem}
\begin{proof}
    From Lemma~\ref{lem:quarter_large_grad}, we know that the number of points with large gradient is at most $T/4$.
    From Lemma~\ref{lem:quarter_saddle} we know that the number of points $\x{t}$ with $\lmin(\nabla^2 f(\x{t})) < -\sqrtra$ is at most $T/4$.
    Hence, at least half of the points are $\alpha$-SOSP.
\end{proof}


